Revisiting Knowledge Distillation: An Inheritance and Exploration Framework

Knowledge Distillation (KD) is a popular technique to transfer knowledge from a teacher model or ensemble to a student model. Its success is generally attributed to the privileged information on similarities/consistency between the class distributions or intermediate feature representations of the teacher model and the student model. However, directly pushing the student model to mimic the probabilities/features of the teacher model to a large extent limits the student model in learning undiscovered knowledge/features. In this paper, we propose a novel inheritance and exploration knowledge distillation framework (IE-KD), in which a student model is split into two parts - inheritance and exploration. The inheritance part is learned with a similarity loss to transfer the existing learned knowledge from the teacher model to the student model, while the exploration part is encouraged to learn representations different from the inherited ones with a dis-similarity loss. Our IE-KD framework is generic and can be easily combined with existing distillation or mutual learning methods for training deep neural networks. Extensive experiments demonstrate that these two parts can jointly push the student model to learn more diversified and effective representations, and our IE-KD can be a general technique to improve the student network to achieve SOTA performance. Furthermore, by applying our IE-KD to the training of two networks, the performance of both can be improved w.r.t. deep mutual learning. The code and models of IE-KD will be make publicly available at https://github.com/yellowtownhz/IE-KD.

==> abstract_nips.tex <==
\begin{abstract}
    Distillation, the transfer of knowledge from a powerful large teacher network or ensemble to a small student network,  is a popular technique for network compression. In this work, we introduce, {\em \LowRedistillation{}},
    a new framework to solve the problem of transferring the knowledge from a small network to a large one.
    Previous distillation methods follow the principle of output consistency, by
    mimicking the feature representations or class probabilities of
    other networks or ensemble, while our \LowRedistillation{} is based on a contrary principle, {\em diversity}. 
    %Such framework emphasizes the consistency among the network outputs, that resembles the idea of model ensemble
    %However, simply distilling in the opposite direction would degenerate the performance of the teacher network, as a large network tends to be lazier.
    In particular, \LowRedistillation{} splits the large network into two parts - inheritance and exploration. The
    inheritance part transfers the compactly represented knowledge from the
    small network to the large network, while the exploration part encourages the large network to
    learn features different from the inherited ones.
    %These two counterpart modules serve as high-level constraints that jointly push the teacher network to learn more diversified and effective features. 
    Extensive experiments demonstrate that these two parts can jointly push the large network to learn more diversified and effective features, and our \LowRedistillation{} can be a general technique to improve the performance of the large network. 
    Furthermore, by alternatively iterating the distillation and \LowRedistillation{} processes between
    two networks, the performance of both can be improved.
    %We show that the student network can even surpass the initial teacher network after few iterations.
\end{abstract}


==> experiments_nips.tex <==
We evaluate our method on both classification and detection tasks. For classification, CIFAR and ImageNet datasets are used. For detection, the PASCAL VOC dataset is used.
We compare our \LowRedistillation{} with independent learning and distillation.
In independent learning, both the large and small networks are independently trained from scratch.
In distillation, the large network is trained by transferring knowledge from the pre-trained small network via consistency control.
By comparing with independent learning, we demonstrate that our \LowRedistillation{} is a general method to improve the performance; and by comparing with distillation, we demonstrate that our exploration loss play a key role in enhancing the network features.

%As reviewed in Section \ref{sec:relatedWorks}, all existing works use consistency control to transfer knowledge between networks. Therefore, we have only these two baselines.

\subsection{Datasets and Settings}

CIFAR-10 and CIFAR-100 \cite{krizhevsky2010cifar} consist of $50,000$ training and $10,000$ test images drawn from
$10$ and $100$ classes.
%For data augmentation, we perform horizontal flips and take random crops from images padded by four pixels on each side, filling missing pixels with reflections of the original image.
Networks are trained using SGD with Nesterov momentum. The
initial learning rate is set to $0.1$, the momentum is set to $0.9$, and the mini-batch
size is set to $128$. The learning rate is divided by $10$ at the
$80$th and $120$th epochs. The training process ends at the $160$th epoch.

ImageNet consists of $1.2$M training images and $50$k validation images with $1,000$ classes.
We perform large-scale experiments on ImageNet ILSVRC $2012$ to verify our
potential ability to transfer more complex and detailed information. Networks
are trained for $100$ epochs, and the learning rate begins at $0.1$ multiplied
by $0.1$ at every $30$ epochs.

We apply our method on Single Shot Detector (SSD) \cite{liu2016ssd}.
Networks are trained on a mixture of the PASCAL VOC$2007$ and VOC$2012$ \cite{everingham2015pascal}
\textit{trainval} sets, which are widely used in object detection. The backbone
network in all models is pre-trained using ImageNet. Networks are
trained for $120$k iterations with a batch size of $32$. Detection
performance is evaluated on the VOC $2007$ \textit{test} set.

\paragraph{Implementation Details}
We implement all networks in PyTorch
\cite{paszke2017automatic} and the code will be released later. The ratio of number of input feature maps and number of factor feature maps is set to $2$. We randomly split representations
of the larger network into inheritance and exploration parts, since the parameters of the network are randomly initialized and there is no strong correlation among channels before learning. The weights of both inheritance and exploration loss
are set to $50$ on CIFAR-10, $100$ on ImageNet, and $100$ on PASCAL VOC.

\subsection{Results of the Image Classification}
\label{sec:result_classification}

%In order to verify the effectiveness for large network improvement, we conduct experiments to show the performances of large network before/after knowledge transfer from small network.
Table \ref{tab:cifar10-teacher} shows the Top-$1$
accuracy on CIFAR-10 when various architectures, including
ResNet \cite{he2016deep}, Wide ResNet \cite{zagoruyko2016wide} and VGG
\cite{simonyan2014very},  are used for the small (S) and large (L) network.
First, we use ResNet-20 as S and ResNet-56 as L, that have same number of channels but different blocks. Then, we test different types of residual networks for S and L with ResNet-20 and WRN-40-1. To investigate the effect of the absence of shortcut connections, we further use VGG13 as S and WRN-46-4 as L. To test the applicability for architectures with the same blocks but different channels, we use WRN-16-1 as S and WRN-16-2 as L. The numbers of parameters of these networks are also given in Table \ref{tab:cifar10-teacher}.


The ``Independent'' represents the networks are independently trained from scratch. The ``S distills L'' and ``S
dedistills L'' denote the large networks are trained using distillation
and dedistillation from pre-trained small networks, respectively.
For a fair comparison, we also use factor transfer \cite{Kim2018ParaphrasingCN} for distillation.
From Table \ref{tab:cifar10-teacher} we observe that: 1) for all network architectures, the performance of L using distillation is even worse than that of independent learning, which indicates that transferring knowledge from a small network to a large network by mimicry alone is not effective, and even harmful; 2) dedistillation consistently improves the performance of the large network for all configurations, indicating the effectiveness of the exploration part, and 3) even with only $1/10$ capacity, the small network VGG-13 can still help improve the performance of the large network WRN-46-4.
%This result confirms that our dedistillation mechanism is a very general and effective means of transfer knowledge from small networks to large networks.

\begin{table*}
\centering
\caption{
    Comparison of the Top-1 classification accuracy (\%) on
    CIFAR-10.
    %when the large network is trained via independent learning,  distillation and dedistillation. S: small network. L: large network.
}
\begin{tabular}{cccccc}
    \hline
    \multicolumn{2}{c}{Network Types} & \multicolumn{2}{c}{Independent} & S distills L & S dedistills L \\
    Net S & Net L & Net S & Net L & Net L & Net L \\
    \hline
    ResNet-20 (0.27M) & ResNet-56 (0.85M) & 92.22 & 93.61 & 92.84 & \textbf{94.56} \\
    \hline
    ResNet-20 (0.27M) & WRN-40-1 (0.56M)  & 92.22 & 93.16 & 92.62 & \textbf{94.10} \\
    \hline
    VGG-13 (0.94M)    & WRN-46-4 (10M)    & 94.01 & 95.56 & 95.29 & \textbf{95.76} \\
    \hline
    WRN-16-1 (0.17M)  & WRN-16-2 (0.69M)  & 91.38 & 93.73 & 93.17 & \textbf{94.65} \\
    \hline
\end{tabular}

    \label{tab:cifar10-teacher}
\end{table*}

\begin{table*}
% \centering
\parbox{.48\linewidth}{
    \centering
    \caption{
        Comparison of Top-$1$ and Top-$5$ classification
        accuracy (\%) on ImageNet.
    }
    \begin{tabular}{c|c|cc}
        \hline
        Method & Network & Top-1 & Top-5 \\
        \hline
        \multirow{2}{*}{Independent} & ResNet-18 (S) & 70.09 & 89.32 \\
        & ResNet-34 (L) & 73.27 & 91.43 \\
        \hline
        S distills L   & ResNet-34 (L) & 72.23 & 90.97 \\
        S dedistills L & ResNet-34 (L) & \textbf{74.46} & \textbf{91.94} \\
        \hline
    \end{tabular}
        \label{tab:imagenet-teacher}
        \vspace{-5mm}
    }
\hfill
\parbox{0.48\linewidth}{
    \centering
    \caption{
        Comparison of object detection in mAP on PASCAL VOC2007.
    }
    \begin{tabular}{c|c|c}
        \hline
        Method & Network & mAP \\
        \hline
        \multirow{2}{*}{Independent} & ResNet-18 (S) & 71.61 \\
        & ResNet-50 (L) & 76.79 \\
        \hline
        S distills L   & ResNet-50 (L) & 76.08 \\
        S dedistills L & ResNet-50 (L) & \textbf{77.48} \\
        \hline
    \end{tabular}
        \label{tab:detection-teacher}
        \vspace{-5mm}
    }
\end{table*}

Table \ref{tab:imagenet-teacher} shows the Top-$1$ and Top-$5$ classification accuracy for large-scale image recognition on ImageNet ILSVRC
$2012$ \cite{russakovsky2015imagenet}. Similar to \cite{Kim2018ParaphrasingCN}, we set ResNet-18 as a pre-trained small network and ResNet-34 as an untrained large
network. As can be seen, dedistillation again outperforms others, and distillation degrades the performance of the large network.
In contrast, even for large-scale recognition, dedistillation from the small network (ResNet-18) improves the large network (ResNet-34) with a significant gain (approximately $1.19$\% gain of top-1 accuracy).

\subsection{Results of Object Detection}
\label{sec:result_detection}
We further verify the effectiveness of
dedistillation for detection tasks. We set ResNet-18
as the small network and ResNet-50 as the large network. Both
networks are pre-trained with ImageNet and fine-tuned on PASCAL VOC $2007$. As shown in Table \ref{tab:detection-teacher}, with dedistillation from the small network, the mean average precision (mAP) of the large network is increased from $76.79\%$ to $77.48\%$.
%In this case, our proposed method shows a notable improvement for the large network, and it implies that our method can be applied to any SSD-based object detector.

\begin{table*}[htpb]
    \centering
    \caption{Comparison of top-$1$ accuracy (\%) on CIFAR-100 between DML \cite{Zhang2017DeepML} and our method.
    }
    \begin{tabular}{ccccccccc}
        \hline
        \multicolumn{2}{c}{Network Types} &  \multicolumn{2}{c}{Independent} &
        \multicolumn{2}{c}{DML} & \multicolumn{2}{c}{Mutual Dedistill} \\
        Net S & Net L & Net S & Net L & Net S & Net L & Net S & Net L \\
        \hline
        ResNet-32 & ResNet-110 & 68.99 & 73.09 & 71.31 & 74.41 & \textbf{72.14} & \textbf{75.51} \\
        \hline
        ResNet-32 & WRN-28-10  & 68.99 & 78.69 & 70.73 & 78.96 & \textbf{72.44} & \textbf{79.87} \\
        \hline
        ResNet-32 & MobileNet  & 68.99 & 73.65 & 71.10 & 76.13 & \textbf{72.17} & \textbf{77.26} \\
        \hline
        ResNet-32 & ResNet-32  & 68.99 & 68.99 & 70.75 & 71.19 & \textbf{71.91} & \textbf{72.35} \\
        \hline
    \end{tabular}
    \label{tab:cifar100-dml}
\end{table*}

\subsection{Extension to Deep Mutual Learning}
\label{sec:exp_mutualTrain}

%In this paper, we pave the way to improve the large teacher network by transferring knowledge from the small student network. A straightforward idea is that we can further improve the student network via a distillation process with the better teacher.
As discussed in Sec. \ref{sec:mutual_learning}, we can alliteratively update the large network by \LowRedistillation{} and the small network by distillation with the improved large network in a deep mutual learning manner \cite{Zhang2017DeepML}, termed \emph{Mutual Dedistill}.
Table \ref{tab:cifar100-dml} compares our Mutual Dedistill with DML \cite{Zhang2017DeepML} on CIFAR-100. DML uses distillation to transfer knowledge in both directions. We experiment on large and small networks with different depths
(ResNet-32/ResNet-110), different widths (ResNet32/WRN-28-10), different building blocks (ResNet-32/MobileNet), and identical
architectures (ResNet32/ResNet32). In all cases, Mutual Dedistill shows clear better improvement than DML and independent learning.
This implies that the small network can also benefit significantly from the improved large network and our dedistillation is complementary to existing distillation/mutual learning methods.

%Specifically, we can iterate the following three steps until converge: a) update the predictions of student and teacher for input mini-batch. b) for small student network, compute the stochastic gradient w.r.t.  supervised loss and distillation loss (e.g. KL distance of output probabilities in \cite{Zhang2017DeepML}) and update its parameters. c) for large teacher network, compute the stochastic gradient w.r.t.  supervised loss and dedistillation loss (described in Sec. \ref{sec:dedistill}) and update its parameters.
% \textbf{CIFAR-10}
% \begin{table*}[htpb]
    % \centering
    % \begin{tabular}{cccccccc}
        % \hline
        % \multicolumn{2}{c}{Network Types} &  \multicolumn{2}{c}{Independent} &
        % \multicolumn{2}{c}{DML} & \multicolumn{2}{c}{Mutual Dedistill} \\
        % Net S & Net T & Net S & Net T & Net S & Net T & Net S & Net T \\
        % \hline
        % ResNet-20 (0.27M) & ResNet56 (0.85M) & 92.22 & 93.61 & 93.15 & \textbf{93.63} & \textbf{94.61} \\
        % \hline
        % ResNet-20 (0.27M) & WRN-40-1 (0.56M) & 92.22 & 93.16 & 93.15 & \textbf{93.47} & \textbf{94.17} \\
        % \hline
        % VGG-13 (0.94M) & WRN-46-4 (10M) & 94.01 & 95.56 & 95.16 & \textbf{95.25} & \textbf{95.83} \\
        % \hline
        % WRN-16-1 (0.17M) & WRN-16-2 (0.69M) & 91.38 & 93.73 & 92.36 & \textbf{92.72} & \textbf{94.75} \\
        % \hline
    % \end{tabular}
    % \caption{
        % Top-1 accuracy (\%) on the CIFAR-10 dataset. ``T distills S''
        % represents distilling from teacher to student.
    % }
    % \label{tab:cifar10-dml}
% \end{table*}
%In addition to distillation methods, our method is also related to deep mutual learning (DML) \cite{Zhang2017DeepML}, which uses distillation loss in a bi-directional way.
%As described in Sec.\ref{sec:mutual_learning}, we extend our method to a mutual learning framework by replacing the distillation loss of the small-to-large direction with dedistillation loss and training both networks from scratch, named as Mutual Dedistill.
%Following \cite{Zhang2017DeepML},

%transferring knowledge from a small network to a large one with distillation loss is sub-optimal; in contrast, dedistillation consistently improves the performance of the large network. Moreover, the small network also benefits significantly from the improved large network.
%The ability of dedistillation to improve mutual learning illustrates that dedistillation is a general mechanism for small-to-large network knowledge transfer and can be adopted into any model training algorithm.


% As shown in Fig. , with the iterative distillation and
% \LowRedistillation, both the performance of teacher and student can be
% improved, and the student can also outperform the teacher network. In practise,
% we found that iterating $3$ times is sufficient for both the teacher and
% student network. Even with only $1/4$ parameters, the student help the teacher
% to improve with a large margin ($0.8\%$ w.r.t 6.35\%).

\subsection{Ablation Study}
%In the introduction, we described the need for a large network to mimic the compact representation of a small network, and learn more different and complementary features to improve diversity and generalization.
%To further analyze the necessity and contribution of inheritance and exploration,
%We conduct ablation studies to analyse the effects of  inheritance and exploration parts, as well as different loss metrics.

In Table \ref{tab:ablation_prop}, we show the results of using different proportions of feature channels for inheritance and exploration, tested on different datasets and network architectures. The settings of  ``$0.0 / 1.0$''
and ``$1.0 / 0.0$'' correspond to using either exploration or inheritance only. The result shows that both inheritance and exploration are important, and even division achieves the optimal performance.


\begin{table*}[htpb]
    \centering
    \caption{
        Ablation study with different proportions of inheritance and exploration feature channels.
    }
    \begin{tabular}{c|cc|ccccc}
        \hline
        Dataset & Net S & Net L & $\eta=0.0/1.0$ & $0.3/0.7$ & $0.5/0.5$ & $0.7/0.3$ & $1.0/0.0$ \\
        \hline
        CIFAR-10  & ResNet-20 & ResNet-56 & 92.93 & 94.05 & \textbf{94.56} & 93.88 & 92.84 \\
        \hline
        CIFAR-100 & ResNet-32 & ResNet-110 & 72.89 & 73.97 & \textbf{74.83} & 74.13 & 73.01 \\
        \hline
        ImageNet  & ResNet-18 & ResNet-34 & 72.23 & 73.75 & \textbf{74.46} & 73.81 & 72.20 \\
        \hline
    \end{tabular}
    \label{tab:ablation_prop}
\end{table*}

In Table \ref{tab:ablation_sim}, we show the results of using different similarity metrics for the inheritance and exploration loss. For simplicity, we use ``$L_2$'' to represent $L_2$ distance as similarity metric and its negative counterpart as dis-similarity metric. The results show that no matter what metric is used our dedistillation consistently improves the performance of the large network.

\begin{table*}[htpb]
    \centering
    \caption{
        Ablation study with different metrics (CIFAR-100).
    }
    \begin{tabular}{cc|ccccc|c}
        \hline
        Net S & Net L & $L_1$ & $L_2$ & cos & partial $L_2$ & $L_1$+CKA & Independent \\
        \hline
        ResNet-32 & ResNet-110 & \textbf{74.83} & 74.74 & 74.57 & 74.12 & 73.79 & 73.09 \\
        \hline
    \end{tabular}
    \label{tab:ablation_sim}
\end{table*}

\subsection{How Does Dedistillation Work?}
\label{sec:reasoning}

\textbf{Inheritance.}
\quad
We use layer-wise relevance propagation (LRP) \cite{lrpOverview} to interpret the network
by visualizing which pixels contribute how much to the classification \cite{lrpProof}.
Fig. \ref{fig:exploration} shows different images and their
LRP heat maps from independent learning and \LowRedistillation{} learning.
We find that LRP heat maps of the inheritance channels in dedistillation resemble the heat maps of independent learning, which indicates that the inheritance part mimics the compact features of the small network well.

Furthermore, we use the number of active neurons \cite{activeSubspace} to analyze the redundancy of
internal representations of networks.
%For an intermediate representation, the number of active neurons is the number of directions to which classification loss function $c(x)$ is sensitive.
The more active neurons, the less redundancy the representation contains \cite{activeSubspace}.
The numbers of active neurons in the small network (ResNet-32) and inheritance channels (ResNet-110) are $45$ and $46$, indicating that the inheritance channels contain approximately the same number of active neurons as the small network.
Moreover, the total number of neurons in inheritance channels is only half of that in the small network, which means that the knowledge is represented more compactly by the inheritance component.

\textbf{Exploration.}
\quad
First, we demonstrate that the exploration part can help discover more \textit{discriminative} input patterns via some concrete examples.
In Fig. \ref{fig:exploration_a}, the ``cheetah'' is misclassified as a ``crocodile'' by the independent model, as the model attributes most of its prediction to the tail of the ``cheetah'' that resembles a ``crocodile''. The exploration part of \LowRedistillation{} model discovers new relevant patterns on ears and mouth that are quite discriminative between the ``cheetah'' and ``crocodile'', and helps predict it correctly.
%This phenomenon verifies that exploration helps the network to find some new and effective features for recognition.
Fig. \ref{fig:exploration_b} shows another example, where the independently trained model is confused by the leaf part of a pear image and misclassifies this image as a ``butterfly''.
The exploration part finds negative relevance of the leaf part (indicated by blue color) that pushes
the model to focus more on the pear and less on the leaf.
%This indicates that exploration pushes the model to find input patterns with opposite relevance.
Similar result is shown in Fig. \ref{fig:exploration_c}. More results are presented in the supplementary materials.
%In summary, exploration improves the model on discovering more \textit{discriminative} input patterns, including different and effective ones (i.e. positive) or same but with opposite relevance (i.e. negative).

Second, we measure the similarity between features from the inheritance channels and exploration channels, when L is trained independently or via \LowRedistilling{}.
Centered Kernel Alignment (CKA) is introduced in \cite{cka} as a similarity index to measure the similarity between two representations. A larger CKA denotes a higher similarity between two sets of representations.
For a fair comparison, the independent model and \LowRedistilling{} model are initialized
with the same random seed.
%And the similarity between corresponding channels of inheritance and exploration is measured for both models.
As shown in Fig.  \ref{fig:cka}, the CKA values are smaller for \LowRedistilling{} in the four networks on CIFAR-100. This indicates more diverse features in the \LowRedistilling{} model.

Third, we calculate the number of active neurons for \LowRedistilling{} and independent models.
Fig. \ref{fig:active_neurons} demonstrates that
\LowRedistillation{} model has more active neurons than the independent model. As proved in \cite{activeSubspace}, this means that the features are more efficient.

\begin{figure}[t]
    \centering
    \subfigure[]
    {
        \includegraphics[width=0.3\linewidth]{figs/lrp_p.pdf}
        \label{fig:exploration_a}
    }
    \subfigure[]
    {
        \includegraphics[width=0.3\linewidth]{figs/lrp_n.pdf}
        \label{fig:exploration_b}
    }
    \subfigure[]
    {
        \includegraphics[width=0.3\linewidth]{figs/lrp3.pdf}
        \label{fig:exploration_c}
    }
    \caption{
        Analysis on how exploration works. ``GT'' denotes the ground
        truth class of the image.
    }
    \label{fig:exploration}
\end{figure}

\textbf{Generalization.}
\quad
Similar to \cite{Zhang2017DeepML,DML1,DML2}, we analyze the sharpness of the converged minima of the independent and \LowRedistilling{} models in Fig. \ref{fig:loss_changes}. Usually, sharp minima leads to poorer generalization, while flat minima has better generalization ability\cite{DML1,DML2}. The experiments are conducted on CIFAR-100 using MobileNet. The converged training loss of both models is approximately the same, $0.131$ for dedistilled model and $0.126$ for independent model, which means the depths of the two minima are close.
As we increase the scale of Gaussian noise added to model parameters, the training loss of the independent model increases faster than that of the dedistilled model. This suggests that the dedistilled model has found a much flatter minimum, and it also provides another explanation for the lower generalization loss of the dedistilled model in Fig. \ref{fig:compare_with_distillation_c}.

\begin{figure}[t]
    \centering
    \subfigure[CKA]
    {
        \includegraphics[width=0.3\linewidth]{figs/cka.pdf}
        \label{fig:cka}
    }
    \subfigure[Active neurons]
    {
        \includegraphics[width=0.3\linewidth]{figs/active_subspace.pdf}
        \label{fig:active_neurons}
    }
    \subfigure[Loss changes]
    {
        \includegraphics[width=0.34\linewidth]{figs/loss_changes.pdf}
        \label{fig:loss_changes}
    }
    \caption{
        Comparison of CKA similarity, numbers of active neurons, and loss changes when Gaussian noise is added.
    }
    \label{fig:analysis}
\end{figure}


==> intro_junx.tex <==
Network compression is a common practice when deploying models in scenarios
that computational and storage resources are limited.  Knowledge
distillation is one of the most popular methods for network compression. 
It was first proposed by Hinton et al. \cite{Hinton2015DistillingTK}
to transfer knowledge from a large teacher network (or ensemble) to a small
student network that is easier to deploy. It works by training the student to
predict the target classification labels, as well as mimicking the class
probabilities \cite{Hinton2015DistillingTK} and/or feature representation
\cite{Zagoruyko2016PayingMA,OD,Kim2018ParaphrasingCN} of the teacher, as these features contain additional information about how the teacher tends to generalize \cite{Hinton2015DistillingTK}. 
Other works have extended this idea to distill the hidden features \cite{Romero2015FitNetsHF},
the attention \cite{Zagoruyko2016PayingMA}, the flow \cite{fastop}, and the mutual learning \cite{Zhang2017DeepML}.

The distillation framework emphasizes the consistency among the network outputs (Fig. \ref{fig:compare_with_distillation_a}), and is mainly used to transfer the knowledge from a larger side (either a larger teacher or an ensemble of students) to a smaller side.
Since the small network employs less complex hypotheses, it usually represents the knowledge in a more compact manner and has a better generalization ability \cite{Romero2015FitNetsHF}.
A question is what can we also perform distillation in the opposite direction, so as to improve the generalization ability and performance of the large network?
As shown by Fig. \ref{fig:compare_with_distillation_c}, simply distilling in the opposite direction would even degenerate the performance of the large network, as the large network tends to be lazier in finding efficient and compact features under the same constraints.


%In spite of aforementioned cases for network compression, there are other cases where network expansion is needed. With the rapid development of cloud computing and the hardware computing power, the limitation of computational and storage resources is gradually alleviated. In this case, we may prefer a larger and more powerful network to replace the currently used small network. Especially in the large scale cloud computing scenario, improving the model accuracy with a slight increase of model complexity is acceptable and is becoming more and more important. Therefore, we face the new problem of expanding a well trained but relatively small network to a stronger one. The most straightforward way to build this larger network is training it from scratch. However, this training-from-scratch solution totally neglects the compact knowledge already learned by the existed small network, thus is not the best option. As distillation has shown that it is possible to improve a network with the knowledge from other networks, it is natural to pave a way to improve the larger network with compactly represented knowledge from the relatively smaller pre-trained network.

\begin{figure}[t]
    \centering
    \subfigure[Distillation]
    {
        \includegraphics[width=0.3\linewidth]{figs/kd.pdf}
        \label{fig:compare_with_distillation_a}
    }
    \subfigure[Dedistillation]
    {
        \includegraphics[width=0.3\linewidth]{figs/kdd.pdf}
        \label{fig:compare_with_distillation_b}
    }
    \subfigure[Loss curves]
    {
        \includegraphics[width=0.3\linewidth]{figs/curve.pdf}
        \label{fig:compare_with_distillation_c}
    }
    \caption{
        (a) and (b): comparison between distillation and dedistillation.
        (c): training the larger network via independent learning (training-from-scratch),
        distillation and dedistillation. 
    }
    \label{fig:compare_with_distillation}
\end{figure}

%Although network expansion and network compression handle opposite problems, they face the same problem that how to transfer knowledge from one network to another. The difference is, in network compression the knowledge is transferred from a larger network to a smaller one while in network expansion the knowledge is transferred in the opposite direction, as shown in Fig. \ref{fig:compare_with_distillation}. The key challenge is, directly pushing the large network to mimic the probabilities/features of the small network as in distillation is like fitting a lower order function with a higher order function, leading to an overfitting problem. Therefore, distillation is not suitable for our network expansion problem and it is even worse than the training-from-scratch, as shown in Fig. \ref{fig:compare_with_distillation}(c).
%Similarly, as mutual learning in \cite{Zhang2017DeepML} uses distillation loss
%in a bi-directional way, we argue that the improvement of the larger network in
%mutual learning is sub-optimal. To solve this challenging problem, we need to figure out what is the difference between the knowledge/outputs of a large network and a small network with the same supervised loss, what is the advantage of a small network compared with the large network, and how can we take this advantage as a reference to learn a large network better. 

%According to the observation in \cite{Ba2013DoDN,ModelCompression}, small networks often have sufficient capacity as large networks, but need to learn more efficient features to realize the desired function. Since the small network employs much less complex hypotheses than the larger network, it usually represents the features in a more compact manner \cite{Romero2015FitNetsHF}.
%and has a better generalization ability.
%Consequently, when knowledge is represented in a  more compact way in the small network, the large network on one hand should mimic this compact representation with part of their parameters, to reduce the redundancy of itself, and on the other hand should release other parameters for exploring more different and complementary features, to improve its diversity and generalization ability. Therefore, in this paper we propose a method to train a larger network by transferring knowledge from a small one, termed dedistillation, as shown in Fig. \ref{fig:compare_with_distillation} (a) and (b).

In this work, we propose a novel technical, termed {\em \LowRedistillation{}}, to transfer the knowledge from small to large network.
As illustrated in Fig. \ref{fig:compare_with_distillation_b}, \LowRedistillation{} embodies two contrary principles $-$ {\em consistency} and {\em diversity}.
Consistency ensures that the compact knowledge encoded in the small network are successfully inherited by the large network, while diversity ensures that the large network can explore new features that are complementary to the inherited ones. 
The idea of \LowRedistillation{} is inspired by the theory of heredity in evolution \cite{darwin1859}. Heredity involves inheritance and variation of traits.
Evolution results from natural selection acting on diversity in populations,
which ultimately stems from mutations. There are three key factors for
evolution: 1) inheritance of compact and effective traits from parents coded by
genes; 2) new diversified genes generated from genetic mutations, and 3) natural
selection through stressful environments.
Motivated by this, we split the features of larger network into two parts: one inherits the compact and effective knowledge encoded by factors \cite{Kim2018ParaphrasingCN} from the small network via a consistency/inheritance loss, and the other is pushed to generate different features via a diversity/exploration loss.
The supervised target loss (e.g. classification or object detection) plays the role of natural selection in heredity, guiding the exploration part to converge to diverse yet effective features.
Another closely related motivation for \LowRedistillation{} comes from the exploration of actions in Q-learning \cite{MnihKSGAWR13}, and the popular AlphaGo \cite{alphago}, where half of the actions follows the predictions of the policy network, and the other half are randomly sampled from the rest action space that ensures adequate exploration of the state space. 
%In this way, the program is pushed to learn some new and effective actions for a better generalization ability. 
%Correspondingly, the inheritance part learns from a well-trained compact small model, the exploration part explores new knowledge for better diversity and generalization ability.

[
TODO:
\begin{itemize}
    \item
    Brief the feature diversity experiments. The goal is to convince the reader the diversity learns diverse and useful features.
    
    \item 
    Emphasize our method is general for different tasks, could be combined with different KD methods and achieve SOTA performance. The goal is to convince the reader our \LowRedistillation{} works well.
    
    \item
    Bones, e.g. mention the mutual learning results. The goal is to surprise the reader our work has many applications.
\end{itemize}

]

Overall, dedistillation provides a simple but effective way to transfer
knowledge from small network to large one. The extensive experiments on
classification and detection tasks show that dedistillation consistently improves the
performance of the large network. Surprisingly, we find that by alternatively
updating the small network via distillation and the large network via
dedistillation in a collaborative manner, the performance of both networks are
boosted. Morevoer, our proposed method also achieves better performance
than other existing distillation methods as can be seen in the supplementary
material.

%Furthermore, in the distillation process, if the large teacher network is improved, we can further
%improve the student network via the same distillation process. Thus, how to
%train a more accurate larger model with the same data and a relatively small
%pre-trained network becomes necessary.

%Specifically, the teacher network is trained with two losses: a conventional supervised learning loss, and a dedistillation loss based on consistency and diversity. For dedistillation loss, we divide the teacher network into two even counterpart components $-$ {\em inheritance} and {\em exploration}. Same as the common knowledge transfer problem, the goal of the inheritance part is to mimic the features of the small network. As their features may have different shape and size, we follow the factor-based distillation method \cite{Kim2018ParaphrasingCN} to embed them into the same space for similarity measurement. As a result, the inheritance part is forced to represent the features in a more compact way, due to its halved size.  In contrast, the exploration part is encouraged to learn new features different from the small network. This is achieved by maximizing the difference between corresponding factors of large and small networks.  By complementing and competing with each other, these two constraints not only improve the diversity of the feature set, but also fiercely push the network to converge to a more robust (flatter) minima with better generalisation to test data. The experiments on both classification and detection tasks indicated that our method could consistently improve the performance of the large network.  Surprisingly, we find that by alternatively update the small network by distillation and the large network by \LowRedistillation{} in a mutual learning manner, the performances of both networks are boosted.


%In summary, our contributions include:
%\begin{itemize}
%    \item
%    \CapRedistillation{}: a new framework to inversely transfer knowledge from a small network to a large network, and consistently improve the performance of the large network.
%    \item
%    Feature exploration: a new method to learn more diverse and effective feature sets with the help of a small pre-trained network.
%    \item
%    %Network evolution: b
%    By alternatively iterating distillation and our \LowRedistillation{} between two networks, both of their performance can be gradually improved.
%\end{itemize}



==> intro_nips.tex <==
Network compression is a common practice when deploying models in scenarios
where computational and storage resources are limited.  Knowledge
distillation is one of the most popular methods for network compression.
It was first proposed by Hinton et al.~\cite{Hinton2015DistillingTK}
to transfer knowledge from a large teacher network (or ensemble) to a small
student network that is easier to deploy.  It works by training the student to
predict the target classification labels and mimic the class
probabilities \cite{Hinton2015DistillingTK} and/or feature representation
\cite{Zagoruyko2016PayingMA,OD,Kim2018ParaphrasingCN} of
the teacher, as these features contain additional information about how the
teacher tends to generalize \cite{Hinton2015DistillingTK}.  Other works have
extended this idea to distill the hidden features \cite{Romero2015FitNetsHF},
the attention \cite{Zagoruyko2016PayingMA}, the flow \cite{fastop}, and the mutual learning \cite{Zhang2017DeepML}.

Despite of aforementioned cases for network compression, there are other cases
where network expansion is needed.
%With the rapid development of cloud computing and hardware computing power, the limitation of computational and
%storage resources is gradually alleviated.
%In this case, we may prefer a larger and more powerful network to replace the currently used small network.
Especially in the large-scale cloud computing scenario, improving model accuracy with a slight
increase in model complexity is acceptable and is becoming increasingly important.
Therefore, we face the new problem of expanding a well-trained but relatively small network to a stronger one.
The most straightforward way to build this larger network is training it from scratch.
However, this training-from-scratch solution neglects the compact knowledge already learned by the existing small network. %and thus is not the best option.
Distillation has been demonstrated to improve a network with the
knowledge from other networks, so it is natural to pave a way to improve the larger
network with compactly represented knowledge from the relatively smaller
pre-trained network.

The challenge of knowledge transfer in network expansion is that the knowledge is transferred in the opposite direction - from a small network to a large one,  as shown in Fig. \ref{fig:compare_with_distillation}.
Directly pushing the large network to mimic the
probabilities/features of the small network as distillation is like fitting
a lower-order function with a higher-order function, leading to an underfitting problem, which is even worse than training the large network from scratch, as shown in Fig. \ref{fig:compare_with_distillation}(c). 
% Thus, a new mechanism is needed for knowledge transfer from small network to a large one.

\begin{figure}[t]
    \centering
    \subfigure[Distillation]
    {
        \includegraphics[width=0.3\linewidth]{figs/kd.pdf}
        \label{fig:compare_with_distillation_a}
    }
    \subfigure[Dedistillation]
    {
        \includegraphics[width=0.3\linewidth]{figs/kdd.pdf}
        \label{fig:compare_with_distillation_b}
    }
    \subfigure[Loss curves]
    {
        \includegraphics[width=0.3\linewidth]{figs/curve.pdf}
        \label{fig:compare_with_distillation_c}
    }
    \caption{
        (a) and (b): comparison between distillation and dedistillation.
        (c): training the larger network via independent learning (training-from-scratch),
        distillation and dedistillation.
    }
    \label{fig:compare_with_distillation}
\end{figure}


%Although network expansion and network compression handle opposite problems, they face the same problem of how to transfer knowledge from one network to another.
%The difference is that in network compression the knowledge is transferred from a larger network to a smaller one while in network expansion the knowledge is transferred in the opposite direction, as shown in Fig. \ref{fig:compare_with_distillation}.
%Therefore, distillation is unsuitable for our network expansion problem and is even worse than training the large network from scratch, as shown in Fig. \ref{fig:compare_with_distillation}(c).
%Similarly, as mutual learning in \cite{Zhang2017DeepML} uses distillation loss
%in a bi-directional way, we argue that the improvement of the larger network in
%mutual learning is sub-optimal.
%To solve this challenging problem, we must determine the difference between the
%knowledge/outputs of a large network and a small network with the same
%supervised loss, which is the advantage of a small network compared
%with a large network, and how can we take this advantage as a reference to better learn a large network.

According to the observation in \cite{Ba2013DoDN,ModelCompression}, small networks often have as sufficient capacity as large
networks but represent the features in a more compact manner \cite{Romero2015FitNetsHF}.
%and has a better generalization ability .
Therefore, a large network, on the one hand, should mimic this compact representation with some of their parameters to
reduce the redundancy of itself and, on the other hand, should release other parameters to explore more different
and complementary features to improve its diversity and generalization ability.
Therefore, in this paper, we propose a method to train a larger network by transferring knowledge from a small one, termed \textit{dedistillation}, as shown in Fig. \ref{fig:compare_with_distillation} (a) and (b).


In our dedistillation, the knowledge is transferred by the two principles of consistency and diversity.
Consistency ensures that the compact knowledge encoded in the small network is successfully inherited by the large network.
Diversity ensures that the large network can explore new features that are complementary to the inherited ones.
The motivation of dedistillation comes from the theory of heredity in evolution
\cite{darwin1859}. Heredity involves inheritance and variation of traits.
Evolution results from natural selection acting on diversity in populations,
which ultimately stems from mutations. There are three key factors for
evolution: a) inheritance of compact and effective traits from parents coded by
genes, b) new diversified genes generated from genetic mutations, and c) natural
selection through stressful environments.
Motivated by this, we split the larger network into two parts: one inherits the compact and effective
knowledge encoded by factors from the small network via consistency/inheritance loss, and
the other is pushed to generate different features via diversity/exploration loss.
The supervised task (classification/detection) loss plays the role of natural selection, guiding the
exploration part to converge to diverse yet effective features.
Another closely related motivation for \LowRedistillation{} comes from the exploration of actions in Q-learning \cite{MnihKSGAWR13}, and the popular AlphaGo \cite{alphago}, where half the actions follow the predictions of the policy network, and the other half are randomly sampled from the remaining action space that ensures adequate exploration of the state space.


%Another closely related motivation for dedistillation comes from the exploration of actions in AlphaGo \cite{alphago}. Half of the actions follows the  predictions of the policy network, the other half are randomly sampled from the rest action space.  In this way, the program is pushed to learn some new and effective actions for a better generalization ability.  Correspondingly, the inheritance part learns from a well-trained compact small model, the exploration part explores new knowledge for better diversity and generalization ability.

%Furthermore, in the distillation process, if the large teacher network is improved, we can further
%improve the student network via the same distillation process. Thus, how to
%train a more accurate larger model with the same data and a relatively small
%pre-trained network becomes necessary.

%Specifically, the teacher network is trained with two losses: a conventional supervised learning loss, and a dedistillation loss based on consistency and diversity. For dedistillation loss, we divide the teacher network into two even counterpart components $-$ {\em inheritance} and {\em exploration}. Same as the common knowledge transfer problem, the goal of the inheritance part is to mimic the features of the small network. As their features may have different shape and size, we follow the factor-based distillation method \cite{Kim2018ParaphrasingCN} to embed them into the same space for similarity measurement. As a result, the inheritance part is forced to represent the features in a more compact way, due to its halved size.  In contrast, the exploration part is encouraged to learn new features different from the small network. This is achieved by maximizing the difference between corresponding factors of large and small networks.  By complementing and competing with each other, these two constraints not only improve the diversity of the feature set, but also fiercely push the network to converge to a more robust (flatter) minima with better generalisation to test data. The experiments on both classification and detection tasks indicated that our method could consistently improve the performance of the large network.  Surprisingly, we find that by alternatively update the small network by distillation and the large network by \LowRedistillation{} in a mutual learning manner, the performances of both networks are boosted.

Overall, dedistillation provides a simple but effective way to transfer knowledge from a small network to a large one. Extensive experiments on
classification and detection tasks show that dedistillation consistently improves the
performance of the large network. Surprisingly, we find that by alternatively
updating the small (student) network via distillation and the large (teacher) network via
dedistillation in a mutual learning manner, the performance of both networks are
boosted. In this way, the small network achieves better performance than existing distillation methods and even outperforms the original teacher. Results will be given in the supplementary material.

%In summary, our contributions include:
%\begin{itemize}
%    \item
%    \CapRedistillation{}: a strategy to inversely transfer knowledge from a relatively small network to a large network that is much more powerful. With dedistillation, we can consistently improve the performance of the large network.
%    \item
%    Feature exploration: a new concept to push the network to learn more diverse and efficient feature sets with the help of a small pre-trained network.
%    \item
%    %Network evolution: b
%    By alternatively iterating distillation and our dedistillation between two networks, the performance of both networks are gradually boosted.
%
%\end{itemize}


==> overview.tex <==


\begin{figure*}[htpb]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/framework}
    \caption{The process of \LowRedistilling{}. The teacher network is split into two
    parts. One part inherits the distilled knowledge from the student network, while the other part
    explores for new knowledge which is different from the student network.
    An auto-encoder is utilized to project the features of teacher and student into the same dimension for distance measurement.}
    \label{fig:framework}
\end{figure*}

In this paper, we proposed a simple and effective approach to inversely transfer the knowledge from the student to the teacher network for improving its performance. Normally, this is very challenging since all knowledge the student has is distilled from the teacher and the teacher network has more parameters and stronger representation power than the student. To achieve this goal, we enforce the teacher to explore more things (via an exploration module) besides learning the knowledge from the student (via an inheriting module). Our method, called \LowRedistillation{} (Section~\ref{sec:student2teacher}), is built upon the existing distillation process (Section~\ref{sec:teacher2student}). For simplicity, we explain the \LowRedistillation{} with the factor-based distillation method \cite{Kim2018ParaphrasingCN}. 
However, we would like to clarify that the \LowRedistillation{} could be combined with any other distillation method, such as the attention transfer \cite{Kim2018ParaphrasingCN} and overhaul distillation \cite{OD}.
Thus, the \LowRedistillation{} could be seen as an upgrade to existing distillation methods.




==> relatedWorks.tex <==

In this paper, we focus on knowledge transfer between or among neural networks. All related works follow the pioneering work of knowledge distillation (KD) that emphasizes the principle of consistency, with difference in the networks (e.g. teacher-student, ensemble of students, etc.), outputs (e.g. classification probabilities, features, etc.) and metrics (e.g. $L_1$, $L_2$ loss, KL divergence, etc.).
In contrast, our work introduces another novel and general principle $-$ diversity, that potentially could be combined with the existing works to further improve the performance.
Below, we mainly describe the distillation related works.

KD is firstly proposed by Hinton et al. \cite{Hinton2015DistillingTK} as a method for network compression, which utilizes the class posterior probabilities produced by the teacher network as ``soft targets'' to facilitate the training of student, as the probability distribution contains more information towards generalization. KL divergence has been used as a distance function to measure the gap between the outputs of student and teacher.

FitNet \cite{Romero2015FitNetsHF} extended this idea by using both the outputs and the intermediate hidden features of the teacher as hints to guide and improve the training of the student. 
In subsequent works, more different forms of knowledge were proposed and transferred to the student, such as the attention \cite{Zagoruyko2016PayingMA}, defined as a set of spatial maps encoding on which spatial areas of the input the network focuses most, and the flow \cite{fastop}, calculated as the inner product between features from neighboring layers.

Since the features of the teacher and student may have different shape and size, it requires a way to measure the similarity of their features and to transfer knowledge.
FitNet \cite{Romero2015FitNetsHF} adopted a regressor with additional parameters to map the student hidden layer to the prediction of the teacher hidden layer.
Kim et al. \cite{Kim2018ParaphrasingCN} proposed a factor-based method, in which the auto-encoder was adopted to project the features into `factors' of the same space.
Heo et al. \cite{AB} adopted an activation transfer loss that has the minimum value when
the boundaries generated by the student coincide with those by the teacher, and later proposed a margin ReLU function to change the distillation feature position to the front of ReLU and use a partial $L_2$ distance function to skip the distillation of unnecessary information \cite{OD}. %Additionally, they use margin ReLU to transform teacher features into factors and $1\times1$ convolutional layers for student features.
Our \LowRedistilling{} could be combined with any of these method for similarity measurement.
%Through the experiments, we found the factor-based method \cite{Kim2018ParaphrasingCN} performed best.

Besides network compression, KD could also be used as a technique to improve training performance. For example, the deep mutual learning \cite{Zhang2017DeepML} shows that an ensemble of students could learn collaboratively and teach each other throughout the training process, even without a powerful teacher network.
BAN \cite{BAN} shows that using the exact
same architecture for the teacher and the student boosts the
performance of the student network.
More recently, FFT \cite{Kim2019FeatureFF}, ONE \cite{KD-on-the-fly} and CL \cite{CL} proposed a
consistency control between an ensemble of sub-network classifiers and each sub-network, where each sub-network mutually teaching one another in an online-knowledge distillation manner.
%Our \LowRedistilling{} approach supports a similar mutual learning between student and teacher, but with the extra knowledge from exploration.
Instead of using an extra teacher network or ensemble, self-distillation is also proposed, such as Tf-KD \cite{KD-TF} that utilizes label smoothing regularization as a virtual teacher, and SD \cite{SnapshotKD} that uses snapshot from earlier epochs as teacher model.

